Underwater Human-Robot and Human-Swarm Interaction: A Review and Perspective

There has been a growing interest in extending the capabilities of autonomous underwater vehicles (AUVs) in subsea missions, particularly in integrating underwater human-robot interaction (UHRI) for control. UHRI and its subfield,underwater gesture recognition (UGR), play a significant role in enhancing diver-robot communication for marine research. This review explores the latest developments in UHRI and examines its promising applications for multi-robot systems. With the developments in UGR, opportunities are presented for underwater robots to work alongside human divers to increase their functionality. Human gestures creates a seamless and safe collaborative environment where divers and robots can interact more efficiently. By highlighting the state-of-the-art in this field, we can potentially encourage advancements in underwater multi-robot system (UMRS) blending the natural communication channels of human-robot interaction with the multi-faceted coordination capabilities of underwater swarms,thus enhancing robustness in complex aquatic environments.

==> figures/diver-swarm_figure/diver-swarm.tex <==
\begin{figure}
    \centering
   \begin{tikzpicture}[node distance=2mm]
        \node[inner sep=0pt] (diver) at (0,0)
            {\includegraphics[width=.1\textwidth]{figures/diver-swarm_figure/diver.png}};
        \node [above,align=center](d) at (diver.north){Human Diver};
            
        \node[inner sep=0pt] (masteruav) at (3,0)
            {\includegraphics[width=.1\textwidth]{figures/diver-swarm_figure/master_uav.png}};
            \node [above,align=center] at (masteruav.north){Master UAV};
            
        \draw[->,thick] (diver.east) -- (masteruav.west);
            % node[midway,fill=white] {Principia Mathematica};
        \node[inner sep=0pt] (acoustic) at (4.5,0)
            {\includegraphics[width=.05\textwidth]{figures/diver-swarm_figure/acoustic_signal.png}};
        
        \node[inner sep=0pt] (swarm) at (6,0)
            {\includegraphics[width=.1\textwidth]{figures/diver-swarm_figure/uav_swarms.png}};
            \node [above,align=center] at (swarm.north){Swarm};

    \end{tikzpicture}
    \caption{Suggestive chain of commands between diver and swarms}
    \label{fig:humanswaemdiagram}
\end{figure}

